Can Multisensory Cues in VR Help Train Pattern Recognition to Citizen Scientists?

As the internet of things (IoT) has integrated physical and digital technologies, designing for multiple sensory media (mulsemedia) has become more attainable. Designing technology for multiple senses has the capacity to improve virtual realism, extend our ability to process information, and more easily transfer knowledge between physical and digital environments. HCI researchers are beginning to explore the viability of integrating multimedia into virtual experiences, however research has yet to consider whether mulsemedia truly enhances realism, immersion and knowledge transfer. My work developing StreamBED, a VR training platform to train citizen science water monitors plans to consider the role of mulsemedia in immersion and learning goals. Future findings about the role of mulsemedia in learning contexts will potentially allow learners to experience, connect to, learn from spaces that are impossible to experience firsthand.

==> Streambed.tex <==
\subsection{Making Qualitative Judgments}
Intuitive qualitative judgments scaffold the way we speak, listen, and interpret the world around us, and help researchers describe and evaluate knowledge that is difficult to teach and evaluate procedurally \cite{perreault1989_QualitativeJudgmentNominal}. Unlike quantitative judgments, which split into a sequence of followable steps or rules, qualitative judgments do not have a pronounced answer, but must be weighed within context. Qualitative judgments thus rely on intuitive judgment and heuristics \cite{gilovich2002heuristics} shaped through experiential learning \cite{kerfoot2003learning}\cite{hmelo2007fish}, cyclically fashioned together from multimodal and multisensory information \cite{haverkamp2001application}, interpreted, and interwoven into previous experience \cite{Young:2016}. 

In biology, qualitative judgments rely on biological observations that consist of \textit{noticing phenomena}, \textit{comparing observations to expectations}, and \textit{recording observations} \cite{eberbach2009everyday}. Noticing consists of knowing when to ask questions, and what question to ask (e.g.``what thing am I looking at?''). After noticing, scientists compare observations to internal webs of information \cite{alberdi2000accommodating}. Intuitive pattern recognition comes from past knowledge \cite{crossan1999organizational}, observing and identifying similarities, differences, and opportunities from a wealth of experience, and chunking experiences into a cognitive map \cite{kerfoot2003learning}. 

Teaching qualitative judgments is difficult because they rely on experiences that are subjective, difficult to surface, examine, and explain, and lead decision makers to interpret stimuli differently \cite{crossan1999organizational}. Although difficult to explain, information must be deliberately scaffolded to be effective; experts that make qualitative judgments chunk interconnected ideas into concepts, models, and patterns that allow them to examine and consider judgments fully \cite{warren2005teaching}. Discussing qualitative judgments helps learners form metaphors that link individual intuition with shared interpretation of meaning, and transfer information between familiar and new domains \cite{crossan1999organizational}. 
%features/characteristics

% -Volunteers in Stream habitat usually do Ph and temperature 
% -reserve qualitative judgment for experts
% 	- however benefit of having volunteers do this is…
\subsection{Qualitative Judgments in Stream Monitoring}
Qualitative stream assessment (or water monitoring) allows groups to visually assess habitats in order to monitor and report on the balance between development and environmental protection, and to advocate for land use that protects regional watersheds \cite{barbour1999rapid}. To do this, groups like the Maryland Department of Natural Resources use monitoring to \textit{benchmark long term stream monitoring trends}, examine \textit{impact of land use} on habitat quality and biological diversity, and assess \textit{cumulative impacts }to streams \cite{roth2002biological}. Roth et al. describes the need for cost-effective integration of statewide efforts to inform the public about stream conditions, increase accuracy of stream condition estimates, and reduce the cost of sampling programs \cite{roth2002biological}. Effective monitoring, Roth notes, must resolve issues in field sampling protocols, differences in types of data collected, and discrepancies in stream condition ratings.

\subsubsection{Assessment using the EPA's Rapid Bioassessment Protocol}
Qualitative stream assessment is a domain with a subjective, flawed protocol that contributes to evaluation errors and relies on extensive background knowledge \cite{striner2016streambed}. The focus of this research is on teaching volunteers to understand and interpret the EPA's Rapid Bioassessment Protocol \cite{barbour1999rapid}, a qualitative \textbf{non-experimental }measure of stream conditions shown in figure \ref{fig:Channel}. To make an informed qualitative assessment, judgments would need to be carefully considered, interpreted, and evaluated in light of precise definitions and scales.  In order to make an informed assessment, an evaluator would have to understand the meaning of quality, then consider what quality attributes corresponded to scales values \cite{fowler1995improving}. Qualitative assessments must also consider subjective issues such as how to \textit{evaluate variation within measures}, how to \textit{evaluate related measures}, and how to \textit{interpret and account for the passage of time} \cite{striner2016streambed}.
 
Judging outdoor spaces is markedly difficult because citizen scientists predominantly lack the background and training to make assessments, and are biased by their limited outdoor experiences. Since the protocol is widely used \cite{roth2002biological}, a challenge is to help learners consider and interpret biases without modifying stream monitoring practices. StreamBED VR endeavors to address these issues through percipient VR training that cost-effectively parallels expert biologist learning experiences. 
  
% \textbf{In light of the challenges novices face, }the way that we currently teach non-experts to make scientific judgments about the natural world is deeply flawed \cite{trumbull2005developing}. Current practices struggle to supply learners with enough background, and fail to recognize learners' need to experience, interpret, and practice assessing training related sensory cues  \cite{roth2002biological}.

\begin{figure}
  \includegraphics[width=1\columnwidth]{figures/Channel5}
    \caption{\textit{Channel Alteration}, a qualitative EPA metric that evaluates human impact on stream channels. This metric poses several challenges, including asking monitors to interpret the meaning of ``normal pattern'' streams and subjective time metrics (e.g.``greater than the past 20 years''), and to judge percentages of channel disturbance.}~\label{fig:Channel}
\end{figure}
% VR  allows teachers to recreate a realistic uniform experience that can train learners efficiently

\subsection{Training in VR}
Virtual reality is a multimodal experience that affords users with a sense of presence in a virtual world \cite{McQuiggan:2008:EEV:1357054.1357291} by transferring spatial knowledge. Presence afforded by embodied VR experiences have been found to affect enjoyment, judgment, learning and emotion \cite{cummings2016immersive}\cite{ahn2014short}, making it an ideal medium to immerse and motivate citizen science participants.  Conservation projects have already begun using the affordances of VR. For instance, the \textit{Many Eyes on the Wild} \cite{bednarz2016virtual} project gave experts around the world the ability  to remotely study habits of jaguars in Peru using VR, and \textit{World in a Box} \cite{fibbi2015wobo} allowed  travelers to transfer remote experiences through 360$^{\circ}$ videos. 
 
VR has been used to to train procedural tasks like operating room protocols \cite{seymour2002virtual}\cite{gallagher2004approval} and submarine periscope training \cite{garris2002games}, but has not been used to train qualitative judgment tasks.  Diverging from previous work, this research aims to use VR to \textit{interpret } protocol metrics in context, \textit{determine} key stream areas based on their purpose and function, and to \textit{appraise} stream spaces using previous experiences. 

\section{Divergent Audience Design}
% Research through design methods include generating, refining, and reflecting on multiple solutions \cite{bowser2016cooperative}.
Literature suggests that designers often anchor to initial designs, using them to make subsequent judgments that can hit a \textit{local maximum} \cite{Norman2012}, a point of diminishing returns \cite{Birkett:LocalMaximums}. To overcome local maximums, Norman and Verganti \cite{Norman2012}\cite{Verganti2008} suggest adopting \textit{radical redesign} methods to assess the viability of design paths. Birkett \cite{Birkett:LocalMaximums} suggests that effective radical redesign uses ``creative leaps'' that are based on understanding users and gaining insight from prior tests. Further, Bartzell et al. suggests that in RTD, data aggregation and reflection are closely related \cite{bardzell2016documenting}, and B\o dker argues for flexible and reflexive design processes \cite{BodkerThirdWaveHCI2006}. The following section describes the method we generated to aggregate user feedback from previous studies to organically address our design needs.    

Expert and design feedback sessions revealed the need for clear task scaffolding, compelling storytelling, and realism, but generated debate on the effectiveness of design components. Although the low fidelity design responded to previous session findings, participants found the prototype unclear and inconsistent and struggled to interpret the narrative. To overcome the design's local maximum, this work broadened the problem space by redesigning the prototype for three different audiences: millennials (our primary audience), baby-boomers (\textbf{citizen science's primary audience}), and teenagers. 

Using our findings from the previous section, we first listed \textit{redesign needs} and divided those needs into specific components. Then we listed \textit{design questions} for each component, and \textit{brainstormed solutions} for each question. We\textit{ grouped solutions} into three different designs, roughly \textit{ sketched out} each design, then constructed \textit{low fidelity mockups} for each sketch. Finally, we \textit{received informal feedback} on the designs from members of different audience groups.  

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth,height=5cm]{figures/DivergentCharttest.jpg}
  \caption{Overview of the \textit{divergent audience design process}. Using the process described in the \textit{Divergent Audience Design }section, this radical-redesign method assesses the viability of different audience design paths.}~\label{fig:DivergentChart}
\end{figure*}

\subsection{Organizing Needs and Questions} 
User needs were organized by previous findings on training and feedback, Nielson's heuristics \cite{nielsen199510}, and Preece et al.'s user experience goals \cite{Preece2016interaction}. Each need was divided into a list of questions for the redesign to address. After organizing needs into questions, we brainstormed 3 solutions for each questions. Rather than trying to answer each question outright, each of the three solutions aimed to come up with a distinct way to address the problem space. Detailed in table \ref{tab:DivergentExample}, one design was to design compelling reward mechanisms.  Questions considered what type reward would be appropriate, whether it should be intrinsic or extrinsic, and whether it should lean on narrative or social dynamic. 

\begin{table}
\centering
\begin{tabular}{L{2cm}|L{6cm}}
\hline
\textit{Design Need} & Ensure training tasks are rewarding \\
\hline
\textit{Questions} & \textit{What reward mechanisms make sense in the training context? Should rewards be intrinsic or extrinsic? Should they be couched into narrative or social dynamics?} \\
\hline
\textit{Solution 1} & Rewards as internal narrative discovery. Making assessments helps you uncover clues about what stream space looked like in the past \\
\hline
\textit{Solution 2} & Social reward. You walk around the stream with a friend that you like. As you make correct assessments, they smile at you more, and stand closer \\
\hline
\textit{Solution 3} & Civic Reward. Proving that human impact (e.g. an oil pipeline) has affected the stream. \\ 
\hline
\end{tabular}
\caption{\label{tab:DivergentExample} An example from the divergent design process. The example considers how to reward training tasks with questions and multiple design solutions.}
\end{table}

\subsection{Designing Solutions for Different Audiences}

After ideating over individual solutions, we color-coded and grouped design ideas to engage three distinct audiences: Young adults (14-18), working millennials (22-30), and retirees (55+). While the ultimate goal was to design for one audience, this process helped us consider how each of the design ideas fit into a range of group needs. Citizen science has historically drawn older, more affluent volunteers \cite{bonney2009citizen}, however young adults and millennials are also viable audiences with different needs, interests, and abilities. 

\subsection{Design Sketches and Low Fidelity Prototypes}

After organizing individual solutions by audience, we explored the  feasibility of parallel design features through a series of simple drawings (figure \ref{fig:SketchesMockups}), then mocked up interactive PowerPoint prototypes. Figure \ref{fig:SketchesMockups} shows a sketch and mockups from the \textit{young adult} design, which was driven by social interaction. In the design, learners explored a stream with a avatar friend that casually pointed out important features of the stream. The friend also served as a social reward, smiling and standing closer to the learner when they mastered learning goals. The aesthetics of this design were driven by a bright cartoon style, and help and feedback mechanisms drew insight from the game show, \textit{Who Wants to be a Millionaire}, previously used to promote active learning in classroom settings \cite{MillionaireActiveLearning}.

\subsection{Strengths and Shortcomings of Parallel Designs}
To understand the strengths and shortcomings of the prototypes, we collected feedback on each of the prototypes from domain experts; the young adult prototype was evaluated by a HCI researcher who works with teens, the retiree prototype was assessed a former biologist who works on citizen sciences projects with older volunteers, and the millennial prototype was assessed by several millennials. Due to time constraints, we did not transcribe or code feedback, and explicitly asked for guidance about \textit{social experience}, \textit{learning mechanisms}, and \textit{narrative}.

\textit{Social Experience} The parallel designs explored how to integrate the social mechanism into training, either with an avatar friend guide (\textit{young adults}), a remote expert giving advice over the phone (\textit{retirees}), or with a second learner also exploring the virtual space (\textit{millennials}). Feedback suggested that expertise could prevent learners from feeling independent, so in the combined mockup in figure \ref{fig:Cues}, an unimposing crayfish cues learners to positive and negative qualities of his stream.

\textit{Learning Mechanism} Feedback on the learning mechanism gave us insight into the importance of blending the scaffold structure into training.  

\reversemarginpar
\marginnote{
\begin{figure}
  \includegraphics[width=\marginparwidth]{figures/DivergentExample1.jpg}
  \caption{A design sketch and interaction mockups showing a design aimed at teenagers. The design uses a avatar friend mechanism who acts as a both a friend an expert guide. The friend supports the learner's exploration by highlighting important areas of the stream, discussing how stream characteristics map onto protocol metrics, and using social cues to motivate learners. The interaction mockup also supported learners with a \textit{Who wants to Be a Millionaire} Lifeline system.}
  \label{fig:SketchesMockups}
\end{figure}
}

Since the information scaffolding was vital to learning, the retiree design explicitly organized important cues into hierarchical information tree that learners could reference during assessment. We expected this to be a helpful feature, but learned that making learning structure explicit could hinder learners' abilities to make effective judgments, akin to a teacher showing students her lesson plan before teaching. Instead, feedback suggested that qualitative relationships may be more effectively taught through problem based learning in a faded scaffold \cite{eberbach2009everyday} to allow learners to independently form relationships. 

\textit{Narrative} The pilot study and expert interviews exhibited the importance of internal narrative to making assessments, so the millennial design focused on giving learners the opportunity to experience what virtual streams looked like in the past and future. Feedback also  suggested that \textit{both} personalized narrative and superficial story framework was vital to motivating learner assessment; giving learners a character and reason for monitoring motivated them to develop the internal narratives for assessment tasks. 

% focusing on internal or external narrative, feedback

% \textit{Assessment Metrics} Feedback on the designs gave us valuable feedback on testing learners before training them. Feedback suggested that a short test of learner skills would not only be a useful metric of learning, but would show learners the challenge of making qualitative assessments, since many novice learners are overconfident about their abilities \cite{goldman2014predicting}.

% % \subsection{Combined Mockup}
% % Using iterative feedback from designers and biologists, we integrated the most effective components of the three designs into a combined 

\begin{figure}
  \centering
  \includegraphics[width=1\columnwidth]{figures/Cues}
  \caption{A \textbf{first-person} mockup of a pair of learners exploring stream environment cues together. In addition to cues presented in the environment, learners receive guidance and feedback from a crayfish, who cues them about them to the state of his habitat.}~\label{fig:Cues}
\end{figure}

